Real-time Control of Electric Autonomous Mobility-on-Demand Systems via Graph Reinforcement Learning

Operators of Electric Autonomous Mobility-on-Demand (E-AMoD) fleets need to make several real-time decisions such as matching available vehicles to ride requests, rebalancing idle vehicles to areas of high demand, and charging vehicles to ensure sufficient range. While this problem can be posed as a linear program that optimizes flows over a space-charge-time graph, the size of the resulting optimization problem does not allow for real-time implementation in realistic settings. In this work, we present the E-AMoD control problem through the lens of reinforcement learning and propose a graph network-based framework to achieve drastically improved scalability and superior performance over heuristics. Specifically, we adopt a bi-level formulation where we (1) leverage a graph network-based RL agent to specify a desired next state in the space-charge graph, and (2) solve more tractable linear programs to best achieve the desired state while ensuring feasibility. Experiments using real-world data from San Francisco and New York City show that our approach achieves up to 89% of the profits of the theoretically-optimal solution while achieving more than a 100x speedup in computational time. We further highlight promising zero-shot transfer capabilities of our learned policy on tasks such as inter-city generalization and service area expansion, thus showing the utility, scalability, and flexibility of our framework. Finally, our approach outperforms the best domain-specific heuristics with comparable runtimes, with an increase in profits by up to 3.2x.

==> sections/issues.tex <==

Major concerns:

1. Assumptions are not clearly stated
    - Model formulation (granularity of demand, deterministic price, known travel costs, known travel times)
    - RL (why 2 GCN layers, parametrization of multimodal distribution)
    - experimental setup (e.g., why is it a node learning problem)
    
    - table with inputs/ outputs (add whats known/ deterministic etc.)
    
2. MDP formulation is presented way late and leads to confusion

---- cut this entirely maybe?

3. The optimal problem is not fully presented

4. The inherent stochasticity in our model is not clearly explained 
    - Is the forecast exact? How do we test performance against inexact forecast? Will MPC performance degrade more than RL?


Minor concerns:
1. The MPC oracle nomenclature is poor. Solution: full-horizon optimal control problem
2. Many poorly worded sentences...


Changes to make:

- New narrative
    - Background section (after the introduction to present the MPC formulation in full detail) 
        - We can introduce all notations, and the setup uses in prior works
        - We can have an assumptions subsection to justify them, and explain that many of them are standard ones
        - We will need to show the full time-expanded graph for this formulation (see fig)
    - Problem Formulation section
        - Introduce the sequential decision making approximation
        - Explain the MDP (and say that the environment will do the matching and the rebalancing without going into the details), where the action is to learn rebalancing flows y_{ij}^{t}.
        - End by saying that we seek an RL agent to solve this MDP, with the hope that it learns temporal information
    - RL framework for E-AMoD section
        - Why GNNs can help
        - Get into details on how we construct a graph G (which is a condensed version of the earlier time-expanded graph)
        - Explain the state, action, and transition rules in more detail (introduce the matching and rebalancing optimizations here)
        - Explain the policy and value network architecture
    - Results section
    
- Updated nomenclature for the baselines
    - MPC with rolling horizon
    - Full horizon optimal control

- Explaining the stochasticity part
    - We dont deal with it at all in this paper. All forecasts are assumed to be exact. The only advantage of a rolling horizon approach is that the runtime improves
    - Future work: Evaluating with uncertainty
    
- New Experiments
    - Beyond 5 node experiments. Train on larger networks
    - Test generalizability across graph sizes
    - Evaluate under uncertainty
